Mining API Usage Scenarios from Stack Overflow

We propose a framework to mine API usage scenarios from Stack Overflow. Each task consists of a code example, the task description, and the reactions of developers towards the code example. First, we present an algorithm to automatically link a code example in a forum post to an API mentioned in the textual contents of the forum post. Second, we generate a natural language description of the task by summarizing the discussions around the code example. Third, we automatically associate developers reactions (i.e., positive and negative opinions) towards the code example to offer information about code quality. We evaluate the algorithms using three benchmarks.

==> introTSETechnicalReport.tex <==
%------------------------------------------
\section{Introduction}\label{sec:intro}
%------------------------------------------
APIs (Application Programming Interfaces)
offer interfaces to reusable software
components. The learnability of an API depends on the availability and usefulness of 
learning resources of the API~\cite{Robillard-APIsHardtoLearn-IEEESoftware2009a,Robillard-FieldStudyAPILearningObstacles-SpringerEmpirical2011a,Stylos-MakingAPIsmoreUsable-PhDThesis2009}. 
Unfortunately, despite developers' reliance on API official documentation as a major resource for 
learning and using APIs~\cite{Ponzanellu-Prompter-EMSE2016}, the documentation can often be incomplete, incorrect, obsolete, and not usable~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015}. 

The shortcomings in the official documentation led to the creation and popularity of online developer forums (e.g., Stack Overflow), where developers can ask and answer questions on how to address diverse development tasks that may involve APIs. 
A number of research efforts have focused on integrating information from the forum posts into API official documentation, such as the linking of API types in Javadocs 
to code examples in forum posts~\cite{Subramanian-LiveAPIDocumentation-ICSE2014}, the presentation of
interesting textual contents from Stack Overflow about an API type in 
Javadocs~\cite{Treude-DocumentationInsightsSO-ICSE2016}, etc. (see \sec\ref{sec:relatedWork}). 

While the linking of a code example to an API type in the Javadoc offers greater insights into how the API type can be used than the actual API 
official documentation, this approach 
can be infeasible in the following scenarios: \begin{inparaenum}[\bfseries(1)]
% \item When too many code examples are connected to an API type that is widely used. For example, the Javadoc of any types in the java.util API can become bloated 
% with thousads or even millions of code examples.  
\item When the code examples may be merely using the API type as a utility, but instead the development tasks in the code examples are \it{more specific} to another API.
\item When the usage of a development task may require more than the linking to a code example, such as contextual information on how to use it.
\end{inparaenum}  
     
As a demonstration of the first problem, consider the two usage scenarios presented in \fig\ref{fig:scenario-motivation}. Both of the two usage 
scenarios use multiple types and methods from the java.util API. In addition, the first code example uses the java.lang API. 
However, both scenarios are related to conversion of JSON data to JSON object. As such, 
the two usage scenarios introduce two open source Java APIs to complete the task (Google GSON in scenario 1 and org.json in scenario 2). This focus is easier 
to understand when we look at the textual contents that describe the two usage scenarios. 

As a demonstration of the second problem, consider the reactions to the two usage scenarios in the comments to the answer in \fig\ref{fig:scenario-motivation}. 
Out of the six comments, two (C1, C2) are associated with the first scenario and two others (C3, C4) with the second scenario. The first comment (C1) complains 
that the provided usage scenario for GSON is not buggy in the newer version of the API. The second comment (C2) confirms that the 
usage scenario is only valid for GSON version 2.2.4. The third comment (C3) complains that the conversion of JsonArray using org.json API is a bit buggy, but the 
next comment (C4) confirms that usage scenario 2 (i.e., the one related to org.json API) works flawlessly. Indeed, reviews about APIs can be useful to 
learn about specific nuances and use cases of the provided code examples~\cite{Uddin-OpinerReviewAlgo-ASE2017,Uddin-OpinerReviewToolDemo-ASE2017}.     

\begin{figure}[t]%[!htb]
  \centering
  \vspace{-4mm}
   \hspace*{-.66cm}%
  \includegraphics[scale=.65]{images/intro_motivating_example}
  \vspace{-8mm}
  \caption{How API usage scenarios are discussed in forum posts.
  }
 
  \label{fig:scenario-motivation}
  \vspace{-7mm}
\end{figure}
We present a framework to automatically mine \it{API usage scenarios} from developer forum posts. 
Each scenario consists of four items: \begin{inparaenum}[\bfseries(1)]
\item A code example as discussed in a forum post, 
\item An API about which the code example is provided to address a development task (for example, the API GSON 
for Code Example 1 in \fig\ref{fig:scenario-motivation}),
\item A natural language description of the code example to summarize what the code does, and 
\item A list of reactions as positive or negative opinions from other developers towards the code example.
\end{inparaenum} 

% Our formulation of an API usage scenario is motivated by the concept of ``minimal manual''~\cite{Carroll-MinimalManual-JournalHCI1987a,Cai-FrameworkDocumentation-PhDThesis2000,Rossen-SmallTalkMinimalistInstruction-CHI1990a,Meij-AssessmentMinimalistApproachDocumentation-SIGDOC1992} that 
% promotes \it{task-oriented} documentation. First introduced in 1987, this 
% concept proposes a briefer documentation to coordinate the attention of the users (i.e., developers) to 
% complete the tasks at hand, rather than distracting them with many pages of \it{self-instructing} manuals (discussed more in \sec\ref{sec:relatedWork}). 

Our proposed API usage scenario mining framework works as follows. First, given as input a forum post that consists of a code example,
we automatically link the code example to an API mentioned in the textual contents of the forum post (i.e., 
the code example is provided to discuss a use case of the API). Second, given as input a code example in a forum post that is 
linked to an API mention, we propose an adaptation of the popular TextRank algorithm~\cite{Mihalcea-Textrank-EMNLP2004} to automatically generate a natural language description of the code example 
by summarizing the usage discussions in the forum post. Third, we automatically associate all 
the reactions that developers posted towards the code example in the forum.   

We evaluated our framework by producing three benchmarks, one each for the three algorithms. 
We observed precisions of 0.957, 0.954, and 0.836 
and recalls of 1.0, 0.974, and 0.768 with the linking of a code example to an API mention in the forum posts, the produced summaries, and the association of reactions to the code examples, respectively. We compared the algorithms against a total of eight state of the art baselines. Our algorithms outperformed all the baselines. 

\nd\bf{Contributions.} We make the following major contributions:
\begin{itemize}
\item \bf{Framework.} We propose a framework to automatically mine API usage scenarios 
from developer forum posts. We present three algorithms to \begin{inparaenum}
\item associate a code example with an API mention in the forum posts,
\item generate natural language summary description of the code example, and
\item associate reactions related to the code example as observed in the forum.
\end{inparaenum} We incorporate the framework in our tool to 
search and summarize API usage. %The tool is available online at: [Hidden for blind review]. 
\item \bf{Evaluation.} We create three benchmarks and compare the algorithms using the benchmarks against eight baselines. 
%We share 
%the benchmark datasets with this paper for future research.
\end{itemize}
We advance the state of the art techniques by \begin{inparaenum}
\item Complementing the code example to API linking algorithms in developer forums~\cite{Subramanian-LiveAPIDocumentation-ICSE2014,Dagenais-RecoDocPaper-ICSE2012a} by 
proposing an algorithm to associate the code example to an API mentioned in the forum texts.
\item Proposing an algorithm to associate code examples to the reactions of other developers and an adaptation of the TextRank algorithm to automatically generate natural language description of code examples in forum posts.
\end{inparaenum}
% \roy{Also what are the major technical contributons? I think you contributed in several dimensions?}
% \roy{I feel like the introduction is not showing the motivation and contributions well. Also what is the state of the art? How you are advancing the area? What techniques did you use? Why those? How did you evaluate your techniques? What is their performance against the state of the art}

% Recent studies on API official documentation~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015,Robillard-APIsHardtoLearn-IEEESoftware2009a} confirm that this concept 
% is still valid, such as in API official documentation (e.g., Javadoc) that simply presents API type and method information without 
% providing code examples on how to use those.  
 
% In their surveys of more than 300 Industrial software developers, Uddin and Robillard~\cite{Uddin-HowAPIDocumentationFails-IEEESW2015}
% observed 10 common problems in API official documentation, both content-based (incompleteness, incorrectnees, ambiguities, obsoleteness, etc.) and presentation-based (meaningless 
% structural information, bloated documentation, etc.).   
% 
% 
% 
% In their seminal work on minimal documentation, Caroll et al. observed that 
% traditional form of API official documention (e.g., Javadoc) is often not useful, 
% because the format often does not conform to specific development needs. For example, 
% developers tend to learn an API by using it in their development tasks. Caroll et al. 
% produced task-based documentation and found that those are more useful than traditional API 
% documentation. 
% 
% 
% 
% 
% While developers consider and expect API official documentation as the major resource 
% to learn and use an API, the official documentation can be often incomplete, incorrect, and 
% obsolete. Useful programs keep changing, proposed as law of program evluation dynamics by 
% Belady and Lehman~\cite{BeladyLehman-ModelLargeProgramDevelopment-IBM1976}.  
% 
% The lack of proper documentation can be a deciding factor for developers during their 
% selection of an API as well. In fact, Uddin and Robillard found that incompleteness of the official 
% documentation can often motivate developers to search for competing APIs. Unfortunately, 
% producing documentation can be often time consuming and devoid of resources, thereby making it 
% unmaintained. This
% observation leads to the question of how we can improve API documentation. 
% 
% 
% 
% The question is now how we can assist in such task-based API usage documentation. One solution 
% would be to ask the API authors to produce such documentation. However, due to the nature of open source APIs, 
% the authors may not have time or resources to produce or maintain such resources. One potential way
% is to produce API documentation by leveraging the crowd, by linking Stack
% Overflow posts with reference
% documentation~\cite{Subramanian-LiveAPIDocumentation-ICSE2014}.
% 
% 
% The online developer forums are interesting avenues for majority of developers
% to look for solutions of their development
% tasks~\cite{Ponzanellu-Prompter-EMSE2016}.
% 
% 
% 
% 
%  Modern-day rapid software development is often facilitated
% by the plethora of open-source APIs available for any given development
% task. The online development portal GitHub~\cite{website:github} now hosts more
% than 67 million public repositories. We can observe a radical increase from the 2.2
% million active repositories hosted in GitHub in 2014. While many of the public repositories in
% GitHub may not be code-based or are personal projects, we observed similar growth in many
% other online API package managers. For example, we observed an increase in the number of open-source APIs
% shared in all the following package managers (as of July 2018) : \begin{inparaenum}
% \item 11,782\% for Javascript APIs in {\em npm} package manager (from 5,646 in December 2011),
% %\item 334\% for Java APIs in online {\em maven} central (from 55,785 in March 2013),
% \item 2,447\% for C\# APIs in online {\em nuget} repository (from 4,799 in February 2012),
% \item 1,477\% for Python APIs in {\em PyPI} (from 9,362 in March 2010).
% \end{inparaenum} Javascript, Java, C\# and Python are among the top five most popular programming
% languages in Stack Overflow\footnote{We used the GitHub API and modulecounts.com to
%  collect the statistics}. Developers can share their APIs in other package managers as well, such as {\em Bower} for Javascript,
%  {\em Rubygems.org} for Ruby, etc.
% 
% % 
% % 
% % By leveraging APIs, developers can benefit from
% % the \it{reusing} of already implemented API features over the
% % \it{re-invention} or \it{re-implementation} of those features. Such benefits can
% % thus increase \it{productivity} and improve the \it{quality} of the
% % software~\cite{Ekwa-APIExplorer-ECOOP2011a}.
% % 
% % Modern day rapid software development is often facilitated by the plethora of
% % open-source APIs that can be available for any given development task. 
% % The online development portal GitHub~\cite{website:github} now hosts more
% % than 67 million active repositories, a radical 
% % increase from the 10 million active repositories in 2013.  
% % Developers share their projects and APIs
% % via other portals as well, e.g., Ohloh~\cite{website:ohloh},
% % Sourceforge~\cite{website:sourceforge}, Freecode~\cite{website:freecode},
% % Maven Central~\cite{website:maven-central}, and so on.
% %  For example, Ohloh currently indexes more than 650,000 API projects,
% %  demonstrating an increase of 100,000 projects from 2015. 
% % \footnote{We used GitHub and
% % Ohloh (Black duck) APIs to generate the statistics.} 
% % Between July 2013 and July 2017, the number of Java artifacts
% % hosted in the online Maven Central repository has increased from a little over
% % 50,000 to around 225,000 (around 350\%
% % increase)~\cite{website:maven-central-growth}.
% 
% Developers can face two major challenges due to the
% abundance of such APIs:
% \begin{description}%[style = nextline]
%   \item [Selection.] Identifying an API amidst choices to support the
%   development task in hand.
%   \item [Usage.] Once an API is selected, a developer would
%   also need to properly learn and use the API.
% \end{description}
% To learn to use an API, the official documentation is provided. Unfortunately, 
% 
% The online developer forums are interesting avenues for majority of developers
% to look for solutions of their development
% tasks~\cite{Ponzanellu-Prompter-EMSE2016}.
% While developer forums serve as communication channels for discussing the
% implementation of the API features, they also enable the exchange
% of opinions about the features. In
% \fig\ref{fig:scenario-motivation}, we show an example usage scenario for the API Google GSON from Stack
% Overflow~\cite{website:so-5554217}. The accepted answer is among the top voted posts in Stack Overflow (score 694) \circled{1}. 
% However, the first comment to the
% post is about the incompatibility of the code example for a new version of
% GSON \circled{2}. The second comment clarifies that the code example works for
% GSON version 2.4.  Indeed, Uddin et al.~\cite{Uddin-SurveyOpinion-TSE2017} observed that developers
% considered the combination of API code examples and API reviews (i.e.,
% reactions) as a form of API documentation, e.g., \emt{You can see how code really
% works, as opposed to how the documentation thinks it works}.
% % \begin{figure}[t]%[!htb]
% %   \centering
% %   \includegraphics[scale=.37]{images/motivation-intro-ase/motivation.png}
% %   \vspace{-6mm}
% %   \caption{How API usage scenarios are discussed in forum posts.
% %   }
% %   
% %   \label{fig:scenario-motivation}
% %   \vspace{-7mm}
% % \end{figure}
% % 
% % 




==> results.tex <==
%%------------------------------------------
%\section{Results}\label{sec:empirical-study}
%%------------------------------------------
%In this section, we answer the research questions.
%\nd We now answer the three research questions below.
%In this section, we answer the research questions.
%\section*{Precision of Mining Usage Scenarios (RQ1)}
%To report performance, we use benchmark-based studies. We generate three separate benchmarks and compare our three algorithms in the mining framework against 
%a set of baselines.
\subsection*{RQ$_{1}$: Performance of the Algorithm to Link Code Example to API Mention}\label{sec:results-performance-linking}
%A high accuracy is required to ensure that code examples are properly
% linked~\cite{Subramanian-LiveAPIDocumentation-ICSE2014}. 
\subsubsection*{\bf{$\bullet$ Approach}} We assess the performance of our algorithm using a benchmark. The benchmark
consists of randomly selected 730 code examples from our entire dataset.
375 code examples were
sampled from the 8589 valid code snippets and 355 from the
4826 code examples that were labeled as
invalid by the \emph{invalid code detection} component of our framework.
The
size of each subset (i.e., valid and invalid samples) is determined to capture a statistically
significant snapshot of our entire
dataset (with a 95\% confidence interval). The evaluation corpus was manually
validated by three independent coders: The first two coders are the first two
authors of this paper, respectively. The third coder is a graduate student and is not a
co-author of this paper.
%The third coder was not involved in any stages of this project.
%For each code example, the final decision
%is taken based on the majority votes out of the three coders.
% Recall
% from \sec\ref{sec:framework} that our algorithm to detect invalid code example
% was based on the rules originally proposed by Dagenais and
% Robillard~\cite{Dagenais-RecoDocPaper-ICSE2012a}. An invalid code in Opiner is
% blob of text that does not have any code (e.g., an XML or JSON block). Note that
% a valid code can still have an XML or JSON string. A valid code can also have
% typos (e.g., in class or variable names). We observed many well-received (e.g.,
% upvoted) code examples to have typos in Stack Overflow.
%
%
%
% A total of three coders contributed to the manual validation process.
% Among the three coders, the first two coders are the first two authors of this
% paper, respectively. The third coder is a graduate student at the University of Saskatchewan.
% The third coder is not a co-author of this paper. The third coder was not
% involved in any stages of this project.
% The first coder did all the tagging.
% The other two coders each assessed approximately 11\% of the 730 code examples
% in the validation dataset (total 80 examples).
The benchmark creation process
involved three steps:
\begin{inparaenum}[(1)]
%\begin{description}
  \item The three coders independently judged randomly
  selected 80 code examples out of the 730 code examples: 50 from the valid code
  examples and 30 from the invalidated code examples. 
  %The two types of code examples are detected using the invalid code detection component, which as noted before, is adapted from~\cite{Dagenais-RecoDocPaper-ICSE2012a}.
  %The three coders then independently judged each code
  %example in this set.
%   The relative proportion of valid and
%   invalid code examples was determined based on the presence of
%   valid and invalid code examples in the entire dataset.
%   \item \bf{Initiation.} The three coders then independently judged each code
%   example in the agreement set.
%   first coder removed his labels from the
%   agreement set and created a spreadsheet with two tabs, 50 valid examples in one tab named as `valid' and 30
%   invalid examples in another tab named as `invalid'. The first
%   coder then sent the spreadsheet to the other two coders by email.
%   To avoid bias, the coders did not have any
%   personal or on-line communication during their assessment of the agreement
%   set.
   %An agreement level is computed among the coders (\tbl\ref{tbl:kappa}).
%   We used the following four
%   metrics from the calculator to assess the agreement: \begin{inparaenum}
%   \item Average pairwise percent agreement,
%   \item Fleiss' Kappa~\cite{Fleiss-FleissKappa-PscyhologicalBulletin1971},
%   \item Average pairwise Cohen Kappa~\cite{Cohen-Kappa-EducationalPsy1960}, and
%   \item Krippendorff's $\alpha$.
%   (nominal)~\cite{Krippendorff-ContentAnalysis-SAGE2003}
%   \end{inparaenum}
\item The agreement among the coders was calculated, which was
  near perfect (\tbl\ref{tbl:kappa}): pairwise Cohen $\kappa$ was 96.6\% and the percent agreement was 99.35\%. To resolve disagreements on a given code example, we took the majority vote. 
%   \item \bf{Agreement Assessment.} The coders
%   agreed with each other on their assessment of invalid code examples. The third coder disagreed with others for this
%   valid code example:
% \begin{lstlisting}
% @JsonCreatorResponseWrapper(@JsonProperty("key"), ...)
% \end{lstlisting}
%  The algorithm associated this one line code example to the API Jackson, which
%  the third coder ruled as an error because the code was \it{too short} to make
%  an informed decision. The code example was taken from the Stack Overflow
%  thread~\cite{website:stackoverflow-q13715753} which was titled as ``Jackson
%  Polymorphic Deserialisation\ldots''. Therefore, the code example is
%  indeed related to the Jackson API. We thus took the decisions of the first two coders on this
%  disagreement, i.e., the algorithm was correct to associate the code example to
%  the API Jackson.
 \item Since the agreement level was
 near perfect, we considered that if any of the coders does further manual labeling,
 there is little chance that those labels would introduce any subjective bias
 in the assessment. The first coder then labeled the rest of the code examples.	
 %finished the labeling
 %of the rest of the code examples (i.e., 650 code examples).
 %The manual validation dataset
 %with the assessment of the coders are shared in our online appendix~\cite{website:opinerusagescenariotse-online-appendix}.
\end{inparaenum}
%\end{description}
  \begin{table}[tbp]
\centering
\caption{Analysis of agreement among the coders to validate the association of APIs
to code examples (Using Recal3~\cite{recal3})}
\vspace{-2mm}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrrr}
\toprule
 & \multicolumn{1}{l}{\textbf{Kappa (Pairwise)}} &
 \multicolumn{1}{l}{\textbf{Fleiss}} & \multicolumn{1}{l}{\textbf{Percent}} & \multicolumn{1}{l}{\textbf{Krippendorff's $\alpha$}} \\
 \midrule
\textbf{Overall} & 0.966 & 0.965 & 99.4\% & 0.966 \\
\textbf{Valid} & 0.932 & 0.930 & 98.7\% & 0.931 \\
\textbf{Discarded} & 1.00 & 1.00 & 100\% & 1.00 \\
\bottomrule
\end{tabular}%
}
\label{tbl:kappa}
\vspace{-5mm}
\end{table}
The manual assessment found nine code examples as invalid. For each of those code examples, 
we labeled our algorithm as wrong, i.e., false positives. In the end, the benchmark consisted 
of 367 valid and 364 invalid code examples. 
%\subsubsection{Baseline} 

\nd\bf{Baselines.} We compare our algorithm against two baselines on the valid code examples.

\begin{inparaenum}[\bfseries B1.]
\nd\item\bf{Baker:} As we noted in \sec\ref{sec:relatedWork}, related 
techniques~\cite{Subramanian-LiveAPIDocumentation-ICSE2014,Phan-StatisticalLearningFQNForums-ICSE2018,Dagenais-RecoDocPaper-ICSE2012a} 
find full qualified names of the API elements in the code examples. Therefore,
if a code example contains code types from multiple APIs, 
the techniques link the code example with all of those APIs. We compare our algorithm 
against Baker, because it is the state of the art technique to leverage an API database in the linking 
process (unlike API usage patterns~\cite{Phan-StatisticalLearningFQNForums-ICSE2018}). 
%As we explained in \sec\ref{sec:intro} (\fig\ref{fig:scenario-motivation}), 
%this approach may not be optimal to link a code example to an API mention about which the code example is discussed in a forum post.
We compare Baker as follows. 
\begin{inparaenum}
\item Code example consisting of code Types Only from one API: We attempt to link it using 
the technique proposed in Baker.
\item Code example consisting of code types from more than one API: if the code example is associated 
to one of the API mentions in the post, we leave it as `undecided' by Baker. We do not penalize 
Baker in such cases, because Baker is not designed to link a code example to an API mention.
\end{inparaenum} 

\nd\item\bf{Search:} Because search engines are predominantly used in development activities involving API usage~\cite{Ekwa-StudyUnfamiliarAPIs-ICSE2012}, 
we search each code example in the online search engine Google. While assessing the search results, 
we check the first three hits (without advertisement). If at least one of the hits contains a reference to the 
associated API, we label the result as correct. We do not consider a search result 
as relevant if it points to the same Stack Overflow post where the code example is found. 
\end{inparaenum}
 \begin{table}[t]
  \centering
\caption{Performance of association of code examples to API Mentions}
\vspace{-2mm}
    \begin{tabular}{l|rrrr}\toprule
    \textbf{Proposed Algorithm} & \multicolumn{1}{l}{\textbf{Precision}} & \multicolumn{1}{l}{\textbf{Recall}} & \multicolumn{1}{l}{\textbf{F1 Score}} & \multicolumn{1}{l}{\textbf{Acc}} \\
    \midrule
    \textbf{Detect Invalid} & -  & -  & -   & 0.969 \\
    \textbf{Link to Valid w/Partial info} & 0.938  & 1.0  & 0.968   & 0.938 \\
    \textbf{Link to Valid w/Full info} & 0.957  & 1.0  & 0.978   & 0.957 \\
    \textbf{Overall w/Partial Info} & 0.938  & 0.969  & 0.953   & 0.953 \\
    \textbf{Overall w/Full Info} & 0.957  & 1.0  & 0.978   & 0.957 \\
    \midrule
    \multicolumn{4}{l}{\bf{Baselines (applied to valid code examples)}} \\
    \midrule
\bf{B1. Baker} & 0.973 &  0.486  &  0.646 & 0.477 \\
%\bf{B2. Popularity} &&&& \\
% \bf{B3. Popularity - D} &&&& \\
% \bf{B4. Popularity - S} &&&& \\
% \bf{B5. Popularity - U+D} &&&& \\
% \bf{B6. Popularity - U+S} &&&& \\
% \bf{B7. Popularity - D+S} &&&& \\
% \bf{B8. Popularity - U+D+S} &&&& \\
\bf{B2. Search (Google)} &  0.389 &  0.881 & 0.539 & 0.369 \\
    \bottomrule
    \end{tabular}%
 \label{tbl:association-accuracy}
 \vspace{-5mm}
\end{table}%
 
\subsubsection*{\bf{$\bullet$ Results}} We achieved a precision of 0.957 and a recall of 1.0 using our algorithm ( \tbl\ref{tbl:association-accuracy}).
A recall of 1.0 was achieved due to greedy approach of algorithm to attempt to find an association for each code example. 
%In general, precision is a more reliable indicator 
%to link code examples to APIs in forum posts~\cite{Subramanian-LiveAPIDocumentation-ICSE2014}.  
The baseline Baker shows the best precision among all (0.973), but with the lowest recall (0.486). This level of precision 
corroborates to the precision reported by Baker on Android SDKs~\cite{Subramanian-LiveAPIDocumentation-ICSE2014}. The low 
recall is due mainly to the inability of Baker to link a code example to an API mention, when more than 
one API is used in the code example. The Google search results show the lowest precision (0.389), confirming 
the assumption that Google is primarily a generally purpose search engine. 

We report the performance of our algorithm under different settings: \begin{inparaenum}
\item \bf{Detect Invalid.} We observed an accuracy of 0.969 to detect invalid code examples.
\item \bf{Link to valid with Partial Info.} We are able to link a valid code to an API mention with a precision of 0.938 using only the type-based filter from the proximity learning and probabilistic learning. 
This experimentation was conducted to demonstrate how much performance we can achieve with minimal information about the candidate APIs. 
Recall that the type-based filter only leverages API type names, unlike a combination of API type and method names (as used by API fully qualified name inference techniques~\cite{Subramanian-LiveAPIDocumentation-ICSE2014,Dagenais-RecoDocPaper-ICSE2012a,Phan-StatisticalLearningFQNForums-ICSE2018}.
\item \bf{Link to valid with Full Info.} When we used all the filters under proximity learning, the precision level was increased to 0.957 to link a valid code example to an API mention. The slight 
improvement in precision confirms previous findings that API types (and not methods) are the major indicators for such linking~\cite{Subramanian-LiveAPIDocumentation-ICSE2014,Dagenais-RecoDocPaper-ICSE2012a}.
\item\bf{Overall.} We achieved an overall precision of 0.938 and a recall of 0.969 while using partial information. 
\end{inparaenum} 


Almost one-third of the misclassified associations happened due to the code
example either being written in programming languages other than Java or the
code example being invalid. The following JavaScript code snippet was
erroneously considered as valid. It was then assigned to a wrong API.
\begin{lstlisting}
var jsonData; $.ajax({type: 'POST', dataType: 'json'})
\end{lstlisting} 
% In our future work,
% we will improve the detection approach of invalid code examples.

Five of the misclassifications occurred due to the code examples being
very short. Short code examples lack sufficient
API types to make an informed decision.  
Misclassifications also occurred due to the API mention detector not being able
to detect all the API mentions in a forum post. For example, the following code
example~\cite{website:stackoverflow-20374351} was erroneously 
assigned to the \api{com.google.code.gson} API. However, the correct association would be the
\api{com.google.gwt} API. The forum post (answer id 20374750) contained both API mentions. However, \api{com.google.gwt} was
mentioned using an acronym GWT and the API mention detector missed it.
\begin{lstlisting}
String serializeToJson(Test test) {
AutoBean<Test> bean = AutoBeanUtils.getAutoBean(test);
return AutoBeanCodex.encode(bean).getPayload();} 
\end{lstlisting}
% Obviously, a higher
% precision is possible if we were to match a code example against all
% code elements in our database~\cite{Subramanian-LiveAPIDocumentation-ICSE2014,Dagenais-RecoDocPaper-ICSE2012a}.
% However, this approach is prone to scalability issues, due mainly
% to the querying of the code types against the entire database. With our database as the Maven public
% repository, we respected their rate limit to ensure the fair usage
% policy. 
% %online public repository
% 
% % In our dataset, 88\% of the association occurred based on the `Global' filter,
% % followed by the `same post before' (9.3\%), `same post after' (1.4\%), 
% % and `same thread' (1.1\%) filters. 
% The Global filter assigns a code example to the API with the maximum type
% match based on the other filters. This filter was the useful when
% API names were not mentioned in the textual contents. In those cases, 
% developers assumed that other developers would automatically infer that
% information. For example, the API \api{org.json} is the default pre-packaged API
% in the Android SDKs. It can be trivial for an Android developer to infer that
% the referenced API is the \api{org.json} API. 
% In \tbl\ref{tbl:association-accuracy}, we show the performance of the 
% filters using the proximity heuristics. The `Global'
% filter has the most coverage, but the lowest precision. This
% mainly happened for short code examples with generic type names. 
% For example, `JsonObject' is a common type name
% among the APIs offering Json Parsing. If a code example only
% contained a reference to this type and nothing else, our coverage rule would
% associate the code example to the org.json API. This was wrong for the following
% code example~\cite{website:stackoverflow-7141650}, because it was
% referring to the \api{com.google.gwt} API:
% \begin{lstlisting}
% JSONObject json_data  = JSONParser.parseLenient(json_string);
% JSONObject data = json_data.get(data).isObject();
% \end{lstlisting}

% 
% \begin{tcolorbox}
% We can associate a code example to an API with 88.3\%
% precision and 98.2\% recall. The misclassifications 
% are due mainly to the greedy approach to associate any code example to
% an API, e.g., one line code example.
% \end{tcolorbox}

%
% Among the association filters, the three filters (Linked, Name, and Dependency)
% showed 100\% accuracy, while Maximum Type Similarity showed slightly higher
% accuracy than the `Coverage' rules\Foutse{rules vs. filters? we need to clarify our terminology!!!}. The Maximum Type Similarity filter was not useful \Foutse{so why do we have it?}, the mention \Foutse{mentioned?} detector did not detect all the potential API mentions. For example, the following code example (thread 20495713) was associated to the
% org.json API, but the org.pubnub API was mentioned in the same thread proximity that the mention \Foutse{mentioned?}
% detector missed:
% \begin{lstlisting}
% public void successCallback(String channel, Object message) {
% JSONObject messageJson = (JSONObject) message;
% }
% \end{lstlisting}
% The invalid code example detector \Foutse{we should italicize the names of these detectors to avoid confusions with other usages of the words in the text!!!}
% showed an accuracy of .99. It incorrectly filtered code examples that did not follow any standard Java syntax (e.g., no semicolon at the end any line). Such code examples often have only one or two lines, e.g., Long.valueOf(mStartTXStr)).
%
%
\subsection*{RQ$_{2}$: Performance of the Summary Description Algorithm}\label{sec:result-summary-desc-informativeness}
%The summary description needs to provide a comprehensive yet concise overview of the code example.
\subsubsection*{\bf{$\bullet$ Approach}} The evaluation of natural language summary description can be conducted in two ways~\cite{Cohan-RevisitingSummarizationEvaluation-LREC2016}: \begin{inparaenum}
\item User study: participants are asked to rate the summaries
\item Benchmark: The summaries are compared against a benchmark.
\end{inparaenum} In benchmark-based settings, 
produced summaries are compared against those in the benchmark using different metrics, 
e.g., coverage and precision of the sentences in the summaries. 
%In rank-based evaluation approaches, the relative position of a sentence in a summary is also 
%considered. In our evaluation, we adopted benchmark-based approach and focused on the precision and recall
%of the produced summaries.

In our previous benchmark (RQ$_1$), a total of 216 code examples were found in the answer posts, i.e., each 
code example is provided in an attempt to suggest a solution to a development task. We assess the performance of our summarization algorithm for those code examples. We create another benchmark by manually producing summary description for the 216 
code examples. To produce the summary description, we used two types of information: \begin{inparaenum}
\item The description of the task that is addressed by the code example, and 
\item The description of the solution as carried out by the code example. 
\end{inparaenum} Both of these information types can be obtained from forum posts, such as problem definition from the question post 
and solution description from the answer post. We picked sentences following principles of extractive summarization~\cite{Cohan-RevisitingSummarizationEvaluation-LREC2016} and minimal manual~\cite{Carroll-MinimalManual-JournalHCI1987a}, i.e., pick only sentences that are related to the task. Consider a task description, ``I cannot convert JSON string into Java object using Gson. I have previously used Jackson for this task." The provided code example is linked to the API Gson. We thus pick the first sentence as relevant to describe the problem, but not the second sentence. A total of two human coders were used to produce the benchmark. The first coder is the first author of this paper. The second coder is a graduate student and is not a co-author of this paper. The two coders followed the following steps:, \begin{inparaenum}
\item Create a coding guide to determine how summaries can be produced and evaluated,
\item Randomly pick $n$ code examples out of the 216 code examples,
\item Produce summary description of each code example, one for the task, i.e., problem (from question post) and one for the provided solution (from answer post).
\item Compute the agreement between the coders. Resolve disagreements by consulting with each other.
\item Iterate the above steps until the coders agreed on at least 80\% of the description in two consecutive iterations, i.e., after that any of the coders can produce the summary description of the rest of code examples without introducing potential individual bias. 
\end{inparaenum} In total, the two coders iterated three times and achieved at least 82\% agreement in two iterations (see \tbl\ref{tab:agreementSummDesc}). In  \tbl\ref{tab:agreementSummDesc}, the number besides an iteration shows the number of code examples that were analyzed by both coders in an iteration (e.g., 30 for the third iteration). On average, each summary in the benchmark contains 5.4 sentences and 
155.5 words.

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
  \centering
  \caption{Percent agreement between the coders for RQ2 benchmark}
  \vspace{-2mm}
    \begin{tabular}{lrrr}\toprule
          & \textbf{Iteration 1 (5)} & \textbf{Iteration 2 (15)} & \textbf{Iteration 3 (30)} \\
          \midrule
    \textbf{Problem} & 60.0\% & 77.8\% & 87.1\% \\
    \textbf{Solution} & 60.0\% & 87.5\% & 83.3\% \\ \midrule 
    \textbf{Overall} & 60.0\% & 82.5\% & 85.2\% \\
    \bottomrule
    \end{tabular}%
  \label{tab:agreementSummDesc}%
   \vspace{-5mm}
\end{table}%

\nd\bf{Baselines.} We compare against four off-the-shelf extractive 
summarization algorithms~\cite{Gambhir-SurveyTextSummarization-JAI2017}:
%\footnote{We used the Python 
%sumy API for the implementation of the algorithms}. 
\begin{inparaenum}[ (B1)]
\item Luhn,
\item Lexrank,
\item TextRank, and
\item Latent Semantic Analysis (LSA).
\end{inparaenum} The first three algorithms 
were previously used to summarize API reviews~\cite{Uddin-OpinerReviewAlgo-ASE2017}. The LSA algorithms are commonly used in information retrieval and software engineering both 
for text summarization and query formulation~\cite{Haiduc-QueryReformulations-ICSE2013}. 
Extractive 
summarization techniques are the most widely used automatic summarization algorithms~\cite{Gambhir-SurveyTextSummarization-JAI2017}. Our proposed algorithm utilizes the TextRank algorithm. Therefore, by applying the TextRank algorithm without the adaption we proposed, we can estimate the impact of the 
proposed changes in algorithm. 



 \begin{table}[t]
  \centering
\caption{Performance of algorithms to produce summary description}
\vspace{-2mm}
    \begin{tabular}{l|rrrr}\toprule
    \textbf{Techniques} & \multicolumn{1}{l}{\textbf{Precision}} & \multicolumn{1}{l}{\textbf{Recall}} & \multicolumn{1}{l}{\textbf{F1 Score}} & \multicolumn{1}{l}{\textbf{Acc}} \\
    \midrule
    \textbf{Proposed Algorithm} & 0.963  & 0.983   &  0.967    &  0.976 \\
%     \textbf{Selective+Eucledian} &   &    &   &  \\
%     \textbf{Selective+Manhattan} &   &    &   &  \\
%     \textbf{Full+Cosine} &   &    &   &  \\
%     \textbf{Full+Eucledian} &   &    &   &  \\
%     \textbf{Full+Manhattan} &   &    &   &  \\
    \midrule
  %  \multicolumn{4}{l}{\bf{Baselines}} \\
  %  \midrule
\bf{B1. Luhn} & 0.656 & 0.823 & 0.713 & 0.766 \\
\bf{B2. Textrank} & 0.659 & 0.826 & 0.716 & 0.768 \\
\bf{B3. Lexrank} & 0.642 & 0.810 & 0.701 & 0.756 \\
\bf{B4. LSA} & 0.646 & 0.816 & 0.705 & 0.760 \\
%\bf{B4. SumBasic} &&&& \\
%\bf{B5. Reduction} &&&& \\
    \bottomrule
    \end{tabular}%
 \label{tbl:description-accuracy}
 \vspace{-5mm}
\end{table}%
\subsubsection*{\bf{$\bullet$ Results}} We achieved the best precision (0.963) and recall (0.983) using 
our proposed engine that is built on top of the TextRank algorithm. 
Each summarization algorithm takes as input the following texts:
\begin{inparaenum}
\item The title of the question, and
\item All the textual contents from both the question and the answer posts.
\end{inparaenum} By merely applying the TextRank algorithm on the input 
we achieved a precision 0.659 and a recall of 0.826 (i.e., without the improvement we suggested in our algorithm). The improvement in our 
algorithm is due to the following two reasons:
\begin{inparaenum}
\item The selection of a smaller subset out of the input texts based on the contexts
of the code example and the associated API (i.e., Step 1 in our proposed algorithm), and 
\item The separate application of our algorithm on the Problem and Solution text blocks. 
This approach was necessary, because the baseline algorithms showed lower recall 
due to their selection of un-informative texts.
\end{inparaenum} 
Out of the four baselines, the TextRank algorithm shows the best performance. 
%The 
%other three algorithms (Luhn, Lexrank, TextRank) show identical performance. 
%The findings 
%offer promises that the production of summary description for a code example from 
%forum posts can be achieved with reasonable success.

\subsection*{RQ$_{3}$: Performance of Linking Reactions to Code Examples}\label{sec:result-link-reaction}
%The reactions about a code example need to be properly linked to the example to show the right usage information.

\subsubsection*{\bf{$\bullet$ Approach}} We assess the performance of our algorithm using a benchmark that is produced by manually associating 
each reaction in the 216 code examples that we analyzed for RQ2. 
Out of the 216 code examples we analyzed in RQ2, the answer posts of 68 code examples consisted of at least one comment. 
In total, 201 comments were posted towards those answers. The comments contained a total of 493 sentences (149 positive, 41 negative). 
A total of three coders manually judged the association of each reaction (i.e., positive and negative sentences) towards the code examples. Each reaction was assessed by at least two coders. The first coder (C1) was the first author, the second (C2) was a graduate student and third (C3) is an undergraduate students. The second and third coders are not co-authors of this paper. The benchmark was produced using the following steps: \begin{inparaenum}
\item We produce a coding guide to evaluate the association of each reaction towards a code example. 
A reaction is associated if it was linked to the code example or the API that was linked to the code example. For example, in \fig\ref{fig:scenario-motivation}, only the first two comments are associated to the code example 1.
%is a positive or a negative comment towards a target entity.  An entity 
%can be the code example, the API mention which is associated to the code example, 
%or another API that may not be related to the code example. 
\item For each reaction, we label it either 1 (associated) or 0 (otherwise). 
\item We compute the agreement between the coders. 
\item We resolve disagreement by assessing the context or taking the majority vote (when possible).
\end{inparaenum}  In \tbl\ref{tab:agreementLinkReaction}, we show the agreement between the coders. The first coder coded all the reactions. The second and third coders coded 152 and 103 reactions, respectively.
%to code   each of the 125 code examples that we used in RQ$_{2}$. A reaction 
%is a positive or a negative comment towards a target entity.  An entity 
%can be the code example, the API mention which is associated to the code example, 
%or another API that may not be related to the code example. We produced the 
%benchmark as follows. \begin{inparaenum}
%\item For each code example, we find the post id in Stack Overflow. Each post 
%is an answer. 
%\item For each answer post, we collect all the comments that are posted in response 
%to the answer. 
%\item For each comment, we label its polarity (positive, negative, or neutral) manually.
%\item For each comment, we detect API mentions in the comment and assign those to 
%the most probable API. 
%\item For each reaction, we label it either 1 or 0. A label of 1 indicates 
%that the comment is related to the code example and a 0 otherwise.
%\end{inparaenum} In total, there were 493 comments posted in response to the 
%125 answers in the benchmark. Out of the 493 comments,  245 are 
%labeled as reactions (average 3.6 per answer post).
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[t]
  \centering
  \caption{Analysis of Agreement Between Coders To Validate the Association of Reactions to Code Examples (Using Recal2~\cite{recal2}}
  \vspace{-2mm}
    \begin{tabular}{lr|rrr}\toprule
          & \textbf{Total}  & \textbf{Percent} & \textbf{Kappa (pairwise)} & \boldmath{}\textbf{Krippendorff’s $\alpha$}\unboldmath{} \\ \midrule
    \textbf{C1-C2} & 152    & 74.5\% & 0.419 & 0.403 \\
    \textbf{C2-C3} & 51    & 62.7\% & 0.117 & 0.052 \\
    \textbf{C1-C3} & 103  & 84.5\% & 0.504 & 0.506 \\
    \bottomrule
    \end{tabular}%
  \label{tab:agreementLinkReaction}%
  \vspace{-5mm}
\end{table}%


\nd\bf{Baselines.} We compare against two baselines:
\begin{inparaenum}[\bfseries B1.]
\item\bf{All Comments.} A code example is linked to all the comments.
\item\bf{All Reactions.} A code example is linked to all the positive and negative comments.
\end{inparaenum} The first baseline offers us insights on how well a blind association technique may 
work, i.e., when we do not consider the proximity of the reactions to the code example. The second 
baseline offers us insights on whether the simple reliance on sentiment detection would suffice.


 \begin{table}[t]
  \centering
\caption{Performance of associating reactions to code examples}
\vspace{-2mm}
    \begin{tabular}{l|rrrr}\toprule
    \textbf{Technique} & \multicolumn{1}{l}{\textbf{Precision}} & \multicolumn{1}{l}{\textbf{Recall}} & \multicolumn{1}{l}{\textbf{F1 Score}} & \multicolumn{1}{l}{\textbf{Acc}} \\
    \midrule
    \textbf{Proposed Algorithm} &  0.836 & 0.768  &  0.794   & 0.878 \\
    \midrule
    \textbf{B1. All Comments} &  0.480 & 0.791   &  0.565    &  0.480 \\
    \textbf{B2. All Reactions} & 0.689  & 0.703  &  0.678   & 0.793 \\
    \bottomrule
    \end{tabular}%
 \label{tbl:reaction-accuracy}
 \vspace{-5mm}
\end{table}%
\subsubsection*{\bf{$\bullet$ Results}} We observed the best precision (0.836) using our proposed algorithm 
and the best recall (0.791) using the baseline All Comments. The baseline `All Reactions' 
shows much better precision than the other baseline, but still lower than our algorithm. 
The lower precision of the `All Reaction' is due to the presence 
of reactions in the comments that are not related to the code example. Such reactions can be 
of two types:
\begin{inparaenum}
\item Developers offer their views of competing APIs in the comments section. Such views also 
generate reactions from other developers. 
%From the usage perspective 
%of a code example, such discussions can be irrelevant. 
%For example, Jackson and GSON are 
%the two most popular APIs, such that the discussion of one of the APIs can bring the reference of 
%another API. 
However, to use the provided code example or complete the development task in hand, 
such discussions are not relevant (e.g., when the code example offers a complete solution). 
\item Developers can also offer views about frameworks that may be using the API associated to the code 
example. For example, some code examples associated with Jackson API were attributed to the 
spring framework, because spring bundles the Jackson API in its framework. We observed that such discussions were often irrelevant, because to use the Jackson 
API, a developer does not need to install the Spring framework. Therefore, from the usage perspective 
of the code example, such reactions are also irrelevant.
\end{inparaenum}
%In \tbl\ref{tbl:reaction-accuracy}, we show the results.
%\subsection{Complementing API Official Documentation (RQ4)}\label{sec:result-link-reaction}



==> resultsComplementOfficialDocumentation.tex <==
%------------------------------------------
\section{RQ$_2$: Usefulness of Mined Scenarios}\label{sec:result-complement}
%------------------------------------------
The mined usage scenarios can improve API documentation, if they offer more
coverage of API usage than the official documentation.
\subsection{Complement API Document with Mined Scenarios (RQ2.1)}

\subsubsection{Approach}
For each of the top five
APIs, we crawled the online Javadocs and official tutorial pages. We found Javadocs for each API. We did not find any
tutorial for three APIs (java.util, org.json, and java.io). For each API, we
computed the coverage of each of the following five API types in the tutorials
(when available) and the mined usage scenarios:
\begin{inparaenum}
\item Class,
\item Interface,
\item Annotation,
\item Exception, and
\item Enum.
\end{inparaenum}

In \tbl\ref{tab:coverage-type-official-mined}, we show the
coverage of the API types in both official documentation and the mined usage
scenarios of the five APIs. For each API and for each of the five API types, the
mined usage scenarios offer more coverage than the official documentation. The
last column in \tbl\ref{tab:coverage-type-official-mined} shows the overall
coverage of the API types in the mined vs official documentation. The overall
coverage is the highest (81.8\%) for the \api{com.google.code.gson} API in the
mined usage scenarios, followed by 62.5\% in the \api{org.json} API. The
\api{org.json} API does not have any official tutorial page.
\begin{table}[t]
\centering
\caption{The coverage of API types in the mined usage scenarios and
in the code examples of API official tutorials (C = Class, I =
Interface, A = Annotation, EX = Exception, EN = Enum) }
\vspace{-2mm}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llrrrrr|r}\toprule
{\textbf{API}} & \textbf{Resource} & {\textbf{C}}
& {\textbf{I}} & {\textbf{A}} & {\textbf{EX}}
& {\textbf{EN}} & {\textbf{Total}} \\
\midrule
\multirow{2}[0]{*}{\textbf{java.util}} & Official & 0     & 0     & -     & 0     & -     & 0 \\
& Mined & 22.22 & 5.26  & -     & 5     & -     & 14.9 \\
\midrule
\multirow{2}[0]{*}{\textbf{org.json}} & Official & 0     & 0     & -     & 0
& -     & 0 \\
& Mined & 57.14 & 100   & -     & 100   & -     & 62.5 \\
\midrule
\multirow{2}[0]{*}{\textbf{gson}} & Official & 28.57 & 75    & 0     & 25    & 0     & 33.33 \\
& Mined & 85.71 & 87.5  & 50    & 100   & 66.67 & 81.82 \\
\midrule
\multirow{2}[0]{*}{\textbf{jackson}} & Official & 1.72  & 0     & 0     & 0     & 20    & 2.21 \\
& Mined & 5.81  & 4.08  & 34.15 & 44.44 & 12    & 8.5 \\
\midrule
\multirow{2}[0]{*}{\textbf{java.io}} & Official & 0     & 0     & -     & 0     & -     & 0 \\
& Mined & 50.98 & 8.33  & -     & 18.75 & -     & 37.98 \\
\bottomrule
\end{tabular}%
}
\vspace{-5mm}
\label{tab:coverage-type-official-mined}%
\end{table}%

The two Java official APIs (java.util and java.io) are more of utility types,
e.g., memory-based collection management of disk-based I/O operations. The APIs
are not specifically designed for JSON-based features. However, they are among
the top five APIs, because any JSON-based task may need to perform such
utility-based operations besides the core task (e.g., JSON parsing).
Intuitively, the usage scenarios for the two APIs can be mined from other
threads besides our dataset. Therefore, the coverage of types for the two APIs
could potentially be much higher in the mined usage scenarios, had we mined all
the Stack Overflow threads tagged as `Java'.

The \api{com.fasterxml.jackson} API have the lowest coverage (8.5\%) in the
mined scenarios. One reason for this is that \api{com.fasterxml.jackson} is the largest API among
the five APIs in terms of the number of API types. The API has a total of 589
types (465 classes, 49 interfaces, 41 annotations, 25 enums and 9 exceptions).
In contrast, the \api{org.json} API has only 16 types (14 classes, 1 interface
and 1 exception). Therefore, it may happen that developers in our dataset did
not need to use all of 589 types of the Jackson API. Indeed, Sawant and
Bacchelli~\cite{Sawant-FineGrapeAPIUsageExtractor-EMSE2016} observed that most
of the features of an API in Github acturally remain unused by the developers.
Another possible reason for the lower coverage is that we may have missed the
discussions of this API in other posts that we did not mine. Our dataset
consists of all the threads tagged as `Java+JSON'. Not all the Stack Overflow
threads discussing the usage of the API are tagged as `Java+JSON'. For example,
the thread (id 27952472) is tagged as `Jackson+java-time'.

\begin{tcolorbox}
For the top five APIs, the mined usage scenarios offer more
coverage for the different API types than the official documentation. The
coverage can be improved by mining more posts from Stack Overflow.
\end{tcolorbox}
\subsection{Impact of Reactions towards Scenarios
(RQ2.2)}\label{sec:results-syntax-errors}
A strong negative reaction towards code examples with syntax errors can be used
as a motivation to avoid those examples during the mining. On the contrary, a code example with synax errors
that is considered useful can still be mined and used for subsequent processing (e.g.,
live API documentation~\cite{Robillard-OndemandDeveloperDoc-ICSME2017})


%The trends remain similar
%across all the APIs.

\begin{table}[t]
  \centering
  \caption{The distribution of syntax errors  in the code examples and
  developers' reactions to the posts containing those examples}
  \vspace{-2mm}
    \begin{tabular}{rlrr|rr}\toprule
          &       & \multicolumn{2}{c}{\bf{With Syntax Error}} &
          \multicolumn{2}{c}{\bf{No Syntax Error}} \\
          \cmidrule{3-6}
          &       & \multicolumn{1}{r}{\bf{Overall}} &
          \multicolumn{1}{r}{\bf{Top 5}} & \multicolumn{1}{r}{\bf{Overall}} &
          \multicolumn{1}{r}{\bf{Top 5}} \\
          \midrule
    \multicolumn{1}{l}{\bf{Snippet}} & Total & 2574  & 1885  & 6022  & 3311 \\
          & Percent & 29.9\% & 21.9\% & 70.1\% & 38.5\% \\
          \midrule
    \multicolumn{1}{l}{\bf{Lines}} & Avg & 2.2   & 2.4   & 6.6   & 8.2 \\
          & Max   & 35    & 35    & 283   & 283 \\
          & STD   & 2.7   & 3.1   & 9.3   & 11.2 \\
          \midrule
    \multicolumn{1}{l}{\bf{Post Score}} & Avg & 2.1   & 1.8   & 2.3   & 1.9
    \\
          & Max   & 187   & 51    & 291   & 58 \\
          & STD   & 6.8   & 3.4   & 7.4   & 3.5 \\
          & Kourtosis & 475.4 & 68.6  & 813.4 & 57.9 \\
          & Skewness & 18.8  & 6.7   & 23.3  & 6 \\
          \midrule
    \multicolumn{1}{l}{\bf{Post Reaction}} & Avg & 0.5   & 0.5   & 0.5   &
    0.5
    \\
          & Max   & 10    & 7     & 10    & 9 \\
          & STD   & 1.6   & 1.6   & 1.5   & 1.5 \\
          & Kourtosis & 2.8   & 1.6   & 3.5   & 2.9 \\
          & Skewness & 0.4   & 0.2   & 0.4   & 0.4 \\
          \bottomrule
    \end{tabular}%
    \vspace{-7mm}
  \label{tab:syntaxerror-vs-reaction}%
\end{table}%
% \begin{table}[t]
%  %\vspace{-2mm}
%   \centering
%   \caption{The distribution of API aspects discussed in the reactions to posts
%   containing code examples with syntax errors }
%   \vspace{-2mm}
%   \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{lrrrr|rrrr}\toprule
%           & \multicolumn{4}{c}{\textbf{With Syntax Error}} & \multicolumn{4}{c}{\textbf{Without Syntax Error}} \\
%           \cmidrule{2-9}
%           & \multicolumn{2}{c}{\textbf{Positive}} & \multicolumn{2}{c}{\textbf{Negative}} & \multicolumn{2}{c}{\textbf{Positive}} & \multicolumn{2}{c}{\textbf{Negative}} \\
%           \cmidrule{2-9}
%           & {\textbf{Avg}} & {\textbf{STD}} & {\textbf{Avg}} & {\textbf{STD}} & {\textbf{Avg}} & {\textbf{STD}} & {\textbf{Avg}} & {\textbf{STD}} \\
%           \midrule
%     \textbf{Performance} & 1.3   & 0.6   & 1.1   & 0.2   & 1.2   & 0.5   & 1.3   & 0.5 \\
%     \textbf{Usability} & 1.9   & 1.2   & 1.6   & 1     & 1.8   & 1.3   & 1.6   & 1.2 \\
%     \textbf{Document} & 1.1   & 0.3   & 1.1   & 0.2   & 1     & 0.2   & 1     & 0 \\
%     \textbf{Legal} & 1     & 0     & 1     & 0     & 1     & 0     & 1     & 0 \\
%     \textbf{Portability} & 1     & 0     & 1.2   & 0.4   & 1.1   & 0.3   & 1     & 0 \\
%     \textbf{Security} & 1     & 0     & 1     & 0     & 1     & 0     & 1     & 0 \\
%     \textbf{Bug} & 1     & 0     & 1.4   & 0.9   & 1.1   & 0.3   & 1.4   & 0.8 \\
%     \textbf{Community} & 1.2   & 0.4   & 1     & 0     & 1     & 0.2   & 1     & 0 \\
%     \textbf{OnlySenti} & 1.4   & 0.7   & 1     & 0.2   & 1.4   & 0.7   & 1     & 0.3 \\
%     \textbf{Features} & 1.4   & 0.8   & 1.3   & 0.6   & 1.4   & 0.8   & 1.3   &
%     0.6
%     \\
%     \bottomrule
%     \end{tabular}%
%     }
%     \vspace{-5mm}
%   \label{tab:aspect-sentiment-error-code}%
% \end{table}%
\begin{table}[t]
%\vspace{-5mm}
  \centering
  \caption{The p-value and effect size in developer's reactions for the posts
  with errors vs no errors}
  \vspace{-2mm}
    \begin{tabular}{lrr|rr}\toprule
          & \multicolumn{2}{c}{\textbf{Overall}} & \multicolumn{2}{c}{\textbf{Top 5}} \\
          \cmidrule{2-5}
          & \multicolumn{1}{r}{\textbf{p-value}} &
          \multicolumn{1}{r}{\textbf{$\delta$}} &
          \multicolumn{1}{r}{\textbf{p-value}} &
          \multicolumn{1}{r}{\textbf{$\delta$}}
          \\
          \midrule
    \textbf{Score} & 0.135 & -0.03 & 0.394 & -0.02 \\
    \textbf{Reaction} & 0.17  & 0.03  & 0.343 & 0.01 \\
    \textbf{Badness vs Disappointment} & 0.06  & 0.207 & 0.09  & 0.205 \\

    \bottomrule
    \end{tabular}%
  \label{tab:p-value-error}%
  %\vspace{-7mm}
\end{table}%
In
\tbl\ref{tab:syntaxerror-vs-reaction}, we show the distribution of the usage scenarios with and without syntax errors. Overall, 29.9\% code examples in our
dataset contained syntax erorrs (21.9\% in the top five APIs). The ``Lines''
rows in \tbl\ref{tab:syntaxerror-vs-reaction} show the distriubtion of code
lines with or without errors. In the code examples with syntax errors,
the error was seen on average 2.2 lines (standard
deviation 2.7). The posts with only such erroneous code examples
has on average a slightly lower score than the posts with
error-free code examples (2.1 vs 2.2 on average). The average reaction scores of
the developers towards the code examples remain the same despite the presence or
absence of such errors. The kurtosis and skewness values for both buckets are
substantial, i.e., developers exhibit high consensus towards their positive
impact. However, the values are lower for the posts with
such erroneous scenarios than those for the posts with error-free scenarios,
i.e., the consensus seems to be lower towards the erroneous code examples.

% The usability of APIs was consulted more in the reactions related to erroneous
% code examples (see \tbl\ref{tab:aspect-sentiment-error-code}). The developers
% complained about the presence of bugs equally for both
% types of code examples. 
Overall, there is no
statistically signicant difference in the score and reaction of the posts for the two types of
code examples (see \tbl\ref{tab:p-value-error}).

To understand whether the developers are more disappointed towards code
examples with many syntax errors, we determine the \it{badness} of each such
code example as follows:
%\begin{equation*}
$\tr{Badness} = \frac{|\tr{\# Lines with Syntax Error}|}{|\tr{\# All Lines}|}$.
%\end{equation*}
For each post continaing only erroneous code example, we compute the
disappointment of the developers:
%\begin{equation*}
$\tr{Disappointment} = \frac{|\tr{\# Negative Reactions}|}{|\tr{\# Negative +
Positive Reactions}|}$.
%\end{equation*}
We then divide the disappointments into two buckets: one
with Badness score $\le$ 50\% and another with Badness score $>$
50\%. While the difference in disappointment between the two buckets is not
statistically significant, it is close 0.06 (see ``Badness vs Disappoinment''
row in see \tbl\ref{tab:p-value-error}).
\begin{tcolorbox}
Almost 30\% of the code examples contained syntax errors. The developers
still consider those almost as useful as the code examples with no such error (given
post score and reaction as indicators of usefulness). However, developer express
more disappointments towards code examples with many such errors.
\end{tcolorbox}



\subsection{Integrating Mined Scenarios to Official Documentation 
(RQ2.3)}\label{sec:result-summ-needs}
API Documentation efforts will be required, if developers face problems in
developer forums to learn and use APIs. More than 90\% of the APIs in our dataset have code examples discussed in the threads that are not tagged as the API name (see \tbl\ref{tbl:api-summ-needs}). The average discoverability score via the tags is only 4.8\%. This means that a developer who relies on the Stack Overflow tags
to find all the usage examples of an API will miss 95.2\%  of usage examples of all the APIs.

\begin{table}[t]
  \centering
  \caption{Discoverability ($< 100\%$), clones and concepts per APIs}
\vspace{-2mm}
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{lrrrr|rrrr}\toprule
          & \multicolumn{4}{c}{\textbf{Overall}}          &
          \multicolumn{4}{c}{\textbf{Top 5}} \\
          \cmidrule{2-9}
          & \multicolumn{1}{l}{\textbf{API}} & \multicolumn{1}{l}{\textbf{\%}}
          & \multicolumn{1}{l}{\textbf{Avg}}
           & \multicolumn{1}{l}{\textbf{STD}} & \multicolumn{1}{l}{\textbf{Avg}} & \multicolumn{1}{l}{\textbf{Max}} & \multicolumn{1}{l}{\textbf{Min}} & \multicolumn{1}{l}{\textbf{STD}} \\
          \midrule
    \textbf{Discover} & 158   & 90.3\% & 4.8
    & 16.1 & 32.7  & 77.6  & 0     & 33.8 \\
    \textbf{Clones} & 96    & 54.9\% & 11             & 20.3  & 38.8  & 84    & 4     & 29.2 \\
    \textbf{Concepts} & 42    & 24.0\% & 13           & 26.6  & 78    & 122   & 31    & 30.7 \\
    \bottomrule
    \end{tabular}%
    }
    \vspace{-5mm}
  \label{tbl:api-summ-needs}%
\end{table}%
Perhaps, due to the difficulty in the discoverability of API usage scenarios, we
observed many cloned code examples in our dataset. A clone denotes that similar feature of an API is consulted more
than once, demonstrating the needs for such solutions from multiple developers.

We found on
average 11 clones in the code examples of 54.9\% of the APIs.  In
\fig\ref{fig:cloned-usage-scenarios}, we show screenshots of three questions
from Stack Overflow. All the
questions are related to the Google GSON API. Each code snippet in
\circled{2}, \circled{4}, \circled{6} are taken from the
accepted/top-voted answers. The
three questions are almost similar. As such, the code snippets also
provide similar solutions using the same GSON types. However, none of the questions are tagged as
duplicate or recommended as similar by the Stack Overflow community as of now.
A search in Stack Overflow
showed that many questions with similar topics
using the same API were asked as recently as in November 2017 (e.g.,
see~\cite{website:so-47134527}).

Besides clones, developers discussed conceptually similar code
examples of APIs in multiple unrelated posts. The learning of an API suffers when
concepts are scattered in many different
posts/pages~\cite{Uddin-TemporalApiUsage-ICSE2012,Robillard-RepresentingConcern-PhDThesis2003}.

Consider the two code examples for the API Jackson in
\fig\ref{fig:jackson-usage-summaries-concept-motivation}.
The first question is
about a development task involving the deserialization a JSON string from a HTTP response.
The second question is about a task involving
the conversion of a JSON file to XML to be served to a web server.
The two code examples in the accepted answers \circled{2} and \circled{4} use
the same API, \api{com.fasterxml.jackson}. Both use the
same API type \tt{ObjectMapper} for mapping of the JSON fields. Besides
\tt{ObjectMapper}, the solution in \circled{4} uses only one other type of the
same API, \tt{XmlMapper}. The two types are structurally connected, because the
input to \tt{XmlMapper} is first processed through the \tt{ObjectMapper}.
Indeed, the deserialization of a JSON input and its
conversion to an XML can be related tasks during the communication of SOAP
(XML) and REST (JSON)-based web servers (e.g., the developer program
APIs~\cite{website:cpc-developerapi} of the Canada Post).
24\% of APIs in our dataset contained such concepts in multiple unrelated posts.

\begin{figure}[t]%[!htb]
\vspace{-2mm}
  \centering
  \includegraphics[scale=.38]{images/motivation-usage-scenario-summaries-shortened2.png}
  \vspace{-2mm}
  \caption{Cloned usage scenarios for API GSON in Stack Overflow}
  \label{fig:cloned-usage-scenarios}
  \vspace{-5mm}
\end{figure}
\begin{figure}[t]%[th]%[!htb]
  \centering
  \includegraphics[scale=.38]{images/motivation2-jackson-shortened.png}
  \vspace{-2mm}
  \caption{Two questions with relevant usage scenarios involving the API Jackson}
  \label{fig:jackson-usage-summaries-concept-motivation}
  \vspace{-7mm}
\end{figure}
\begin{tcolorbox}
Multiple code examples in 90\% of the APIs
cannot be discovered via the Stack Overflow tags. The code examples of more than 54\% of
the APIs have clones. Conceptually
related code examples are often discussed in multiple unrelated posts for 24\%
of APIs.
\end{tcolorbox}






==> results_ase2019.tex <==
%%%------------------------------------------
%\section{Results}\label{sec:empirical-study}
%%------------------------------------------

%\nd We now answer the four research questions below.

\subsection{RQ$_1$ Performance of Linking Code Example to API Mention}\label{sec:results-performance-linking}
%A high accuracy is required to ensure that code examples are properly
% linked~\cite{Subramanian-LiveAPIDocumentation-ICSE2014}. 
\subsubsection*{\bf{$\bullet$ Approach}} We assess the performance of our algorithm to link code examples to API mentions using a benchmark that
consists of randomly selected 730 code examples from our entire corpus.
375 code examples were
sampled from the 8589 valid code snippets and 355 from the
4826 code examples that were labeled as
invalid by the \emph{invalid code detection} component of our framework.
The
size of each subset (i.e., valid and invalid samples) is determined to capture a statistically
significant snapshot of our entire
dataset (95\% confidence interval). The evaluation corpus was manually
validated by three coders: The first two coders are the first two
authors of this paper. The third coder is a graduate student and is not a co-author.
The benchmark creation process
involved three steps:
\begin{inparaenum}[(1)]
%\begin{description}
  \item The three coders independently judged randomly
  selected 80 code examples out of the 730 code examples: 50 from the valid code
  examples and 30 from the invalid code examples. 
\item The agreement among the coders was calculated, which was
  near perfect (\tbl\ref{tbl:kappa}): pairwise Cohen $\kappa$ was 0.97 and the percent agreement was 99.4\%. To resolve disagreements on a given code example, we took the majority vote. 
 \item Since the agreement level was
 near perfect, we considered that any of the coders could complete the rest of the coding without introducing any subjective bias. The first coder then labeled the rest of the code examples.	
\end{inparaenum}
%\end{description}
  \begin{table}[tbp]
\centering
\caption{Analysis of agreement among the coders to validate the association of APIs
to code examples (Using Recal3~\cite{recal3})}
\vspace{-2mm}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrrr}
\toprule
 & \multicolumn{1}{l}{\textbf{Kappa (Pairwise)}} &
 \multicolumn{1}{l}{\textbf{Fleiss}} & \multicolumn{1}{l}{\textbf{Percent}} & \multicolumn{1}{l}{\textbf{Krippen $\alpha$}} \\
 \midrule
\textbf{Overall} & 0.97 & 0.97 & 99.4\% & 0.97 \\
\textbf{Valid} & 0.93 & 0.93 & 98.7\% & 0.93 \\
\textbf{Discarded} & 1.0 & 1.0 & 100\% & 1.0 \\
\bottomrule
\end{tabular}%
}
\label{tbl:kappa}
\vspace{-2mm}
\end{table}
The manual assessment found nine code examples as invalid. We labeled our algorithm as wrong for those, i.e., false positives. In the end, the benchmark consisted 
of 367 valid and 363 invalid code examples. 
%\subsubsection{Baseline} 

\nd\bf{Baselines.} We compare our algorithm against two baselines on the valid code examples.

\begin{inparaenum}[\bfseries B1.]
\nd\item\bf{Baker:} As we noted in \sec\ref{sec:relatedWork}, related 
techniques~\cite{Subramanian-LiveAPIDocumentation-ICSE2014,Phan-StatisticalLearningFQNForums-ICSE2018,Dagenais-RecoDocPaper-ICSE2012a} 
find fully qualified names of the API elements in the code examples. Therefore,
if a code example contains code types from multiple APIs, 
the techniques link the code example with all of those APIs. We compare our algorithm 
against Baker, because it is the state of the art technique to leverage an API database in the linking 
process (unlike API usage patterns~\cite{Phan-StatisticalLearningFQNForums-ICSE2018}). 
%As we explained in \sec\ref{sec:intro} (\fig\ref{fig:scenario-motivation}), 
%this approach may not be optimal to link a code example to an API mention about which the code example is discussed in a forum post.
We compare Baker as follows. 
\begin{inparaenum}
\item Code example consisting of code Types Only from one API: We attempt to link it using 
the technique proposed in Baker~\cite{Subramanian-LiveAPIDocumentation-ICSE2014}.
\item Code example consisting of code types from more than one API: if the code example is associated 
to one of the API mentioned in the post, we leave it as `undecided' by Baker. 
%We do not penalize 
%Baker in such cases, because Baker is not designed to link a code example to an API mention.
\end{inparaenum} 

\nd\item\bf{Search:} Because search engines are predominantly used in development activities involving API usage~\cite{Ekwa-StudyUnfamiliarAPIs-ICSE2012}, 
we search each code example in Google. While assessing the search results, 
we check the first three hits (without advertisement). If at least one of the hits contains a reference to the 
associated API, we label the result as correct. We do not consider a search result 
as relevant if it points to the same Stack Overflow post where the code example is found. 
\end{inparaenum}
 \begin{table}[t]
  \centering
\caption{Performance of linking code examples to API Mentions}
\vspace{-2mm}
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|rrrr}\toprule
    \textbf{Proposed Algorithm} & \multicolumn{1}{l}{\textbf{Precision}} & \multicolumn{1}{l}{\textbf{Recall}} & \multicolumn{1}{l}{\textbf{F1 Score}} & \multicolumn{1}{l}{\textbf{Acc}} \\
    \midrule
    \textbf{Detect Invalid} & -  & -  & -   & 0.97 \\
    \textbf{Link Valid w/Partial info} & 0.94  & 1.0  & 0.97   & 0.94 \\
    \textbf{Link Valid w/Full info} & 0.96  & 1.0  & 0.98   & 0.96 \\
    \textbf{Overall w/Partial Info} & 0.94  & 0.97  & 0.95   & 0.95 \\
    \textbf{Overall w/Full Info} & 0.96  & 1.0  & 0.98   & 0.96 \\
    \midrule
    \multicolumn{4}{l}{\bf{Baselines (applied to valid code examples)}} \\
    \midrule
\bf{B1. Baker} & 0.97 &  0.49  &  0.65 & 0.48 \\
\bf{B2. Search (Google)} &  0.39 &  0.88 & 0.54 & 0.37 \\
    \bottomrule
    \end{tabular}%
    }
 \label{tbl:association-accuracy}
 \vspace{-2mm}
\end{table}%
 
\subsubsection*{\bf{$\bullet$ Results}} We achieved a precision of 0.96 and a recall of 1.0 using our algorithm (\tbl\ref{tbl:association-accuracy}).
A recall of 1.0 was achieved due to the greedy approach of our algorithm which attempts to find an association for each code example. The baseline Baker shows the best precision among all (0.97), but with the lowest recall (0.49). This level of precision 
corroborates with the precision reported by Baker on Android SDKs~\cite{Subramanian-LiveAPIDocumentation-ICSE2014}. The low recall is due mainly to the inability of Baker to link a code example to an API mention, when more than 
one API is used in the code example. The Google search results show the lowest precision (0.39), confirming 
the assumption that Google is primarily a generally purpose search engine. 

We report the performance of our algorithm under different settings: \begin{inparaenum}
\item \bf{Detect Invalid.} We observed an accuracy of 0.97 to detect invalid code examples.
\item \bf{Link to valid with Partial Info.} We are able to link a valid code to an API mention with a precision of 0.94 using only the type-based filter from the proximity learning and probabilistic learning. 
This experimentation was conducted to demonstrate how much performance we can achieve with minimal information about the candidate APIs. 
Recall that the type-based filter only leverages API type names, unlike a combination of API type and method names (as used by API fully qualified name inference techniques~\cite{Subramanian-LiveAPIDocumentation-ICSE2014,Dagenais-RecoDocPaper-ICSE2012a,Phan-StatisticalLearningFQNForums-ICSE2018}. Out of the two learning rules in our algorithm, Proximity learning shows better precision than Probabilistic learning (2 vs 14 wrong associations). 
\item \bf{Link to valid with Full Info.} When we used all the filters under proximity learning, the precision level was increased to 0.96 to link a valid code example to an API mention. The slight 
improvement in precision confirms previous findings that API types (and not methods) are the major indicators for such linking~\cite{Subramanian-LiveAPIDocumentation-ICSE2014,Dagenais-RecoDocPaper-ICSE2012a}.
\item\bf{Overall.} We achieved an overall precision of 0.94 and a recall of 0.97 while using partial information. 
\end{inparaenum} 


Almost one-third of the misclassified associations happened due to the code
example either being written in programming languages other than Java or the
code example being invalid. The following JavaScript code snippet was
erroneously considered as valid. It was then assigned to a wrong API: \begin{verbatim}
var jsonData; $.ajax({type: `POST'})...
\end{verbatim}
% In our future work,
% we will improve the detection approach of invalid code examples.

Five of the misclassifications occurred due to the code examples being
very short. Short code examples lack sufficient
API types to make an informed decision.  
Misclassifications also occurred due to the API mention detector not being able
to detect all the API mentions in a forum post. For example, the following code
example~\cite{website:stackoverflow-20374351} was erroneously 
assigned to the \api{com.google.code.gson} API. However, the correct association would be the
\api{com.google.gwt} API. The forum post (answer id 20374750) contained both API mentions. However, \api{com.google.gwt} was
mentioned using an acronym GWT and the API mention detector missed it.
\begin{lstlisting}
AutoBean<Test> b = AutoBeanUtils.getAutoBean(test)
return AutoBeanCodex.encode(b).getPayload(); 
\end{lstlisting}
\subsection{RQ$_2$ Performance of Producing Textual Task Description}\label{sec:result-summary-desc-informativeness}
%The summary description needs to provide a comprehensive yet concise overview of the code example.
\subsubsection*{\bf{$\bullet$ Approach}} The evaluation of natural language summary description can be conducted in two ways~\cite{Cohan-RevisitingSummarizationEvaluation-LREC2016}: \begin{inparaenum}
\item User study: participants are asked to rate the summaries
\item Benchmark: The summaries are compared against a benchmark.
\end{inparaenum} In benchmark-based settings, 
produced summaries are compared against those in the benchmark using metrics, 
e.g., precision of the sentences in the summaries. 
%In rank-based evaluation approaches, the relative position of a sentence in a summary is also 
%considered. In our evaluation, we adopted benchmark-based approach and focused on the precision and recall
%of the produced summaries.

In our previous benchmark (RQ$_1$), a total of 216 code examples were found in the answer posts, i.e., each 
code example is provided in an attempt to suggest a solution to a development task. We assess the performance of our summarization algorithm for those code examples. We create another benchmark by manually producing summary description for the 216 
code examples. To produce the summary description, we used two types of information: \begin{inparaenum}
\item the description of the task that is addressed by the code example, and 
\item the description of the solution as carried out by the code example. 
\end{inparaenum} Both of these information types can be obtained from forum posts, such as problem definition from the question post 
and solution description from the answer post. We picked sentences following principles of extractive summarization~\cite{Cohan-RevisitingSummarizationEvaluation-LREC2016} and minimal manual~\cite{Carroll-MinimalManual-JournalHCI1987a}, i.e., pick only sentences that are related to the task. Consider a task description, \emph{``I cannot convert JSON string into Java object using Gson. I have previously used Jackson for this task".} If the provided code example is linked to the API Gson, we pick the first sentence as relevant to describe the problem, but not the second sentence. A total of two human coders were used to produce the benchmark. The first coder is the first author of this paper. The second coder is a graduate student and is not a co-author of this paper. The two coders followed the following steps: \begin{inparaenum}
\item create a coding guide to determine how summaries can be produced and evaluated,
\item randomly pick $n$ code examples out of the 216 code examples,
\item produce summary description of each code example by summarizing the problem text (from question post) and the solution text (from answer post).
\item Compute the agreement between the coders. Resolve disagreements by consulting with each other.
\item Iterate the above steps until the coders agreed on at least 80\% of the description in two consecutive iterations, i.e., after that any of the coders can produce the summary description of the rest of code examples without introducing potential individual bias. 
\end{inparaenum} In total, the two coders iterated three times and achieved at least 82\% agreement in two iterations (see \tbl\ref{tab:agreementSummDesc}). In  \tbl\ref{tab:agreementSummDesc}, the number besides an iteration shows the number of code examples that were analyzed by both coders in an iteration (e.g., 30 for the third iteration). On average, each summary in the benchmark contains 5.4 sentences and 
155.5 words.

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
  \centering
  \caption{Agreement between the coders for RQ2 benchmark}
  \vspace{-2mm}
  \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lrrr}\toprule
          & \textbf{Iteration 1 (5)} & \textbf{Iteration 2 (15)} & \textbf{Iteration 3 (30)} \\
          \midrule
    \textbf{Problem} & 60.0\% & 77.8\% & 87.1\% \\
    \textbf{Solution} & 60.0\% & 87.5\% & 83.3\% \\ \midrule 
    \textbf{Overall} & 60.0\% & 82.5\% & 85.2\% \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:agreementSummDesc}%
   \vspace{-5mm}
\end{table}%

\nd\bf{Baselines.} We compare against four off-the-shelf extractive 
summarization algorithms~\cite{Gambhir-SurveyTextSummarization-JAI2017}:
%\footnote{We used the Python 
%sumy API for the implementation of the algorithms}. 
\begin{inparaenum}[ (B1)]
\item Luhn,
\item Lexrank,
\item TextRank, and
\item Latent Semantic Analysis (LSA).
\end{inparaenum} The first three algorithms 
were previously used to summarize API reviews~\cite{Uddin-OpinerReviewAlgo-ASE2017}. The LSA algorithms are commonly used in information retrieval and software engineering both 
for text summarization and query formulation~\cite{Haiduc-QueryReformulations-ICSE2013}. 
Extractive 
summarization techniques are the most widely used automatic summarization algorithms~\cite{Gambhir-SurveyTextSummarization-JAI2017}. Our proposed algorithm utilizes the TextRank algorithm. Therefore, by applying the TextRank algorithm without the adaption that we proposed, we can estimate the impact of the 
proposed changes on the algorithm. 



 \begin{table}[t]
  \centering
\caption{Algorithms to produce summary description}
\vspace{-2mm}

    \begin{tabular}{l|rrrr}\toprule
    \textbf{Techniques} & \multicolumn{1}{l}{\textbf{Precision}} & \multicolumn{1}{l}{\textbf{Recall}} & \multicolumn{1}{l}{\textbf{F1 Score}} & \multicolumn{1}{l}{\textbf{Acc}} \\
    \midrule
    \textbf{Proposed Algorithm} & 0.96  & 0.98   &  0.97    &  0.98 \\
    \midrule
\bf{B1. Luhn} & 0.66 & 0.82 & 0.71 & 0.77 \\
\bf{B2. Textrank} & 0.66 & 0.83 & 0.72 & 0.77 \\
\bf{B3. Lexrank} & 0.64 & 0.81 & 0.70 & 0.76 \\
\bf{B4. LSA} & 0.65 & 0.82 & 0.71 & 0.76 \\
    \bottomrule
    \end{tabular}%
 \label{tbl:description-accuracy}
 %\vspace{-5mm}
\end{table}%
\subsubsection*{\bf{$\bullet$ Results}} We achieved the best precision (0.96) and recall (0.98) using 
our proposed engine that is built on top of the TextRank algorithm. 
Each summarization algorithm takes as input the following texts:
\begin{inparaenum}
\item the title of the question, and
\item all the textual contents from both the question and the answer posts.
\end{inparaenum} By merely applying the TextRank algorithm on the input 
we achieved a precision 0.66 and a recall of 0.83 (i.e., without the improvement of selecting sentences using beam search that we suggested in our algorithm). The improvement in our 
algorithm is due to the following two reasons:
\begin{inparaenum}
\item the selection of a smaller subset out of the input texts based on the contexts
of the code example and the associated API (i.e., Step 1 in our proposed algorithm), and 
\item the separate application of our algorithm on the Problem and Solution text blocks. 
This approach was necessary, because the baselines showed lower recall 
due to their selection of un-informative texts.
\end{inparaenum} 
The TextRank algorithm is the best performer among the baselines. 

\subsection{RQ$_3$ Performance of Linking Reactions to Code Examples}\label{sec:results-performance-linking-reaction}

\subsubsection*{\bf{$\bullet$ Approach}} We assess the performance of our algorithm using a benchmark that is produced by manually associating reactions towards the 216 code examples that we analyzed for RQ1 and RQ2. 
Out of those 216 code examples, 68 code examples from 59 answers consisted of at least one comment (total 201 comments). 
The 201 comments had a total of 493 sentences (190 positive, 55 negative, 248 neutral). 
Four coders judged the association of each reaction (i.e., positive and negative sentences) towards the code examples. For each reaction, we label it either 1 (associated to the code example) or 0 (non-associated). The association of each reaction to code example was assessed by at least two coders. The first coder (C1) is the first author, the second (C2) is a graduate student, third (C3) is an undergraduate student, and fourth (C4) is the second author of the paper. The second and third coders are not co-authors of this paper. The first coder coded all the reactions. The second and third coders coded 174 and 103 reactions, respectively. For each reaction, we took the majority vote to determine its reaction (e.g., if C2 and C3 label as 1 but C1 as 0, we took 1, i.e., associated). The fourth coder (C4) was consulted when a majority was not possible. This happened for 22 reactions where two coders (C1 and C2/C3) were involved and they disagreed. The labeling was accompanied by a coding guide. \tbl\ref{tab:agreementLinkReaction} shows the agreement among the first three coders.
%
%The benchmark was produced using the following steps: \begin{inparaenum}
%\item we produce a coding guide to evaluate the association of each reaction towards a code example. 
%A reaction is associated if it was linked to the code example to the API that was linked to the code example. For example, in \fig\ref{fig:scenario-motivation}, only the first two comments are associated to the code example 1.
%\item We compute the agreement between the coders (see \tbl\ref{tab:agreementLinkReaction}). \chk{We resolve disagreement by taking the majority vote (when labels from all three coders were available). For 22 sentences, where two coders were involved and they disagreed, we took the labels of C2/C3, who are not co-authors of the paper.}
%\end{inparaenum}  
\begin{table}[t]
  \centering
  \caption{Analysis of Agreement Between Coders To Validate the Association of Reactions to Code Examples (Using Recal2~\cite{recal2})}
  \vspace{-2mm}
  %\resizebox{\columnwidth}{!}{%
    \begin{tabular}{lr|rrr}\toprule
          & \textbf{Total}  & \textbf{Percent} & \textbf{Kappa (pairwise)} & \boldmath{}\textbf{Krippen $\alpha$}\unboldmath{} \\ \midrule
    \textbf{C1-C2} & 174    & 83.9\% & 0.46 & 0.45 \\
    \textbf{C2-C3} & 51    & 62.7\% & 0.12 & 0.05 \\
    \textbf{C1-C3} & 103  & 84.5\% & 0.50 & 0.51 \\
    \bottomrule
    \end{tabular}%
   % }
  \label{tab:agreementLinkReaction}%
  \vspace{-2mm}
\end{table}%


\nd\bf{Baselines.} We compare against two baselines:
\begin{inparaenum}[\bfseries B1.]
\item\bf{All Comments.} A code example is linked to all the comments.
\item\bf{All Reactions.} A code example is linked to all the positive and negative comments.
\end{inparaenum} The first baseline offers us insights on how well a blind association technique that does not leverage sentiment detection may work. The second 
baseline offers us insights on whether the simple reliance on sentiment detection would suffice.


 \begin{table}[t]
  \centering
\caption{Performance of associating reactions to code examples}
\vspace{-2mm}
    \begin{tabular}{l|rrrr}\toprule
    \textbf{Technique} & \multicolumn{1}{l}{\textbf{Precision}} & \multicolumn{1}{l}{\textbf{Recall}} & \multicolumn{1}{l}{\textbf{F1 Score}} & \multicolumn{1}{l}{\textbf{Acc}} \\
    \midrule
    \textbf{Proposed Algorithm} &  0.89 & 0.94  &  0.91   & 0.89 \\
    \midrule
    \textbf{B1. All Comments} &  0.45 & 0.84   &  0.55    &  0.45 \\
    \textbf{B2. All Reactions} & 0.74  & 0.84  &  0.78   & 0.74 \\
    \bottomrule
    \end{tabular}%
 \label{tbl:reaction-accuracy}
 \vspace{-2mm}
\end{table}%
\subsubsection*{\bf{$\bullet$ Results}} We observed the best precision (0.89) and recall (0.94) using our proposed algorithm to link reactions to code examples. The baseline `All Reactions' 
shows much better precision than the other baseline, but still lower than our algorithm. 
The lower precision of the `All Reaction' is due to the presence 
of reactions in the comments that are not related to the code example. Such reactions can be 
of two types:
\begin{inparaenum}
\item Developers offer their views of competing APIs in the comments section. Such views also 
generate reactions from other developers. 
%From the usage perspective 
%of a code example, such discussions can be irrelevant. 
%For example, Jackson and GSON are 
%the two most popular APIs, such that the discussion of one of the APIs can bring the reference of 
%another API. 
However, to use the provided code example or complete the development task using the associated API, such discussions are not relevant. 
\item Developers can also offer views about frameworks that may be using the API associated to the code example. For example, some code examples associated with Jackson API were attributed to the 
spring framework, because spring bundles the Jackson API in its framework. We observed that such discussions were often irrelevant, because to use the Jackson 
API, a developer does not need to install the Spring framework. Therefore, from the usage perspective of the code example, such reactions are irrelevant.
\end{inparaenum}

\subsection{RQ$_4$ Effectiveness of a Task-Centric API Documentation}
%\subsection{Effectiveness of a Task-Based Documentation Tool (RQ$_{4}$)}\label{sec:discussions}
We implemented our framework in an online tool, where a developer can search an
API by its name to see all the mined usage scenarios of the API from Stack
Overflow.
The current version shows results from our evaluation corpus. We present the
usage scenarios in summarized form, e.g., group code examples that use the same
types (e.g., class) of the API. As noted in \sec\ref{sec:case-study}, our
    evaluation corpus uses Stack Overflow 2014 dataset. This choice was not
    random. We wanted to see, given sufficient time, whether the usage scenarios
    in our corpus were included in the API official documentation.
    % In \tbl\ref{tbl:api-resolution-overview}, we show the distribution of the
    % mined scenarios in the corpus.
    We found a total
of 8596 valid code examples linked to 175 distinct APIs in our corpus. The
majority of those (60\%) were associated to five APIs: java.util, org.json,
Gson, Jackson, java.io.
Most of the mined scenarios for those APIs were absent in their official
documentation, e.g., for Gson, only 25\% types are used in the code examples of
its official documentation, but 81.8\% of the types are discussed in our mined
usage scenarios. This finding highlights that even with sufficient time between a usage scenario 
is discussed in forum post, API authors are not including or they do not have sufficient resource to include 
those scenarios from Stack Overflow to API official documentation.
 Therefore, the automatic mining of the usage scenarios using our framework can assist 
the API authors who could not include those in the API official documentation.
% 
% The tool is designed based on two major
% observations:
% \begin{enumerate}[leftmargin=10pt]
%     \item \bf{Documentation Needs}. As noted in \sec\ref{sec:case-study}, our
%     evaluation corpus uses Stack Overflow 2014 dataset. This choice was not
%     random. We wanted to see, given sufficient time, whether the usage scenarios
%     in our corpus were included in the API official documentation.
%     % In \tbl\ref{tbl:api-resolution-overview}, we show the distribution of the
%     % mined scenarios in the corpus.
%     We found a total
% of 8596 valid code examples linked to 175 distinct APIs in our corpus. The
% majority of those (60\%) were associated to five APIs: java.util, org.json,
% Gson, Jackson, java.io.
% Most of the mined scenarios for those APIs were absent in their official
% documentation, e.g., for Gson, only 25\% types are used in the code examples of
% its official documentation, but 81.8\% of the types are discussed in our mined
% usage scenarios.
% 
%     \item \bf{Summarization Needs}. On average each
% of the top five APIs in our corpus is linked to more than 1039 scenarios. We
% found more than 500 code examples for just one class (\tt{ObjectMapper}) from
% Jackson API alone. Thus, a straightforward crowd documentation approach like
% Baker~\cite{Subramanian-LiveAPIDocumentation-ICSE2014}, by annotating the
% Javadoc of an API type with all the mined scenarios may be infeasible. We thus
% needed to produce a \it{summarized} representation of the mined scenarios, e.g.,
% by grouping usage scenarios that use the same API types.
% % , similar to the summarization of API
% % reviews~\cite{Uddin-OpinerReviewAlgo-ASE2017}.
%     % Indeed, we found that the
% % scenarios of 54\% of the APIs have clones (using
% % NiCad~\cite{CKRoy-Nicad-ICPC2008}).
% \end{enumerate}


%\begin{table}[t]
%  \centering
%  \caption{Distribution of Code Snippets By APIs}
%  \vspace{-2mm}
%    \begin{tabular}{rrrr|rrrr}\toprule
%    \multicolumn{4}{c}{\textbf{Overall}} & \multicolumn{4}{c}{\textbf{Top 5}} \\
%    \midrule
%    {\textbf{API}} & {\textbf{Snippet}} 
%    & {\textbf{Avg}} & {\textbf{STD}} 
%    & {\textbf{Snippet}} & {\textbf{Avg}} 
%    & {\textbf{Max}} & {\textbf{Min}} \\
%    \midrule
%    175   & 8596  & 49.1  & 502.7 & 5196  & 1039.2 & 1951  & 88    \\
%    \bottomrule
%    \end{tabular}%
%  \label{tbl:api-resolution-overview}%
%  \vspace{-5mm}
%\end{table}%

%\nd\bf{Research Journey.} The above observations led to the question of how we can improve API documentation. One potential way is by linking Stack
%Overflow posts with reference documentation~\cite{Subramanian-LiveAPIDocumentation-ICSE2014}. 
%Another way is to create a dedicated \it{portal} for APIs, where developers 
%can search for API usage and learn about their pros and cons in a synthesized manner~\cite{Uddin-OpinerReviewAlgo-ASE2017}. To investigate the design of a tool to complement API documentation, we sought to answer the following questions:
%\begin{enumerate}
%\item Are all the mined scenarios useful? 
%\item Can we document the large volume of usage scenarios?
%\end{enumerate}
%The first question is necessary, because a code example in a forum post with many syntactical error may be unusable, while one with minor syntactical error may still be worthy of documentation. We 
%observed that almost 30\% of the mined code examples contained syntax
%errors. The developers still consider those almost as
%useful as the code examples with no such error (given
%post score and reaction as indicators of usefulness).
%However, developer express more disappointments towards code examples with many syntax errors.
%
%The second question is necessary, because the five popular APIs in our dataset have many usage scenarios. Thus, a straightforward representation, such as annotating the Javadoc of an API type with all the mined scenarios may be infeasible. For example, we found more than 500 scenarios for the class \code{ObjectMapper} of Jackson API. Therefore, one possible approach is to \it{summarize} the mined scenarios, similar to the summarization of API reviews~\cite{Uddin-OpinerReviewAlgo-ASE2017}. Indeed, 
%we found that the
%scenarios of 54\% of the APIs have
%clones (using NiCad~\cite{CKRoy-Nicad-ICPC2008}). 
%Moreover, conceptually related code examples (e.g., frequently co-used API types~\cite{Robillard-APIProperty-IEEETSE2012}) are often
%discussed in multiple unrelated posts for 24\% of APIs. 

\begin{figure}[t]%[!htb]
  \centering
  \vspace{-2mm}
  \hspace*{-.6cm}%
  \includegraphics[scale=.7]{images/opiner-intro}
  \hspace*{-.8cm}%
  \vspace{-6mm}
  \caption{Screenshots of our deployed API usage scenario summarizer online tool}
  \label{fig:opiner-intro}
  \vspace{-5mm}
\end{figure}
% \begin{figure}[t]
% \centering
% \vspace{-6mm}
% \hspace*{-.8cm}%
% \includegraphics[scale=1.2]{images/concept-summary}
% \hspace*{-.8cm}%
% \vspace{-4mm}
% \caption{Concept based summary for API Jackson}
% \label{fig:concept-summary}
% \vspace{-4mm}
% \end{figure}
%\nd\bf{Tool.} To facilitate API usage through the mined usage scenarios, we developed an online 
%API usage scenario search and summarization engine. 
In \fig\ref{fig:opiner-intro}, we show screenshots of our tool.
A user can search an API by name in \circled{1} to see the usage summary page of the API in
\circled{3}, where the mined scenarios are presented. An example scenario is shown
in \circled{4}. Other relevant and similar usage scenarios are grouped under 
`See Also' (\circled{5}). Each scenario under the
`See Also' can be further explored (\circled{6}). Each usage scenario is
linked to the corresponding post in Stack Overflow where the code example was
found (by clicking on the \it{details} label). The front page shows the top 10 APIs with the most number of scenarios \circled{2}. 

%\nd\bf{Future Work.} 

\nd\bf{$\bullet$ Effectiveness of our Tool.} Although we extensively evaluated the algorithms of our framework in terms of the evaluation metrics, we also measured the effectiveness of our tool with a user study. We recruited 31 developers (18 professionals) who each completed four coding tasks involving four APIs (one task for each of Jackson~\cite{website:jackson}, Gson~\cite{website:gson}, Spring~\cite{website:spring} and Xstream~\cite{website:xstream}). The objects were four resources (our tool, Stack Overflow, Official documentation, Search Engines). Each task was completed by at least seven participants using each resource. We collected the time took to complete each task. The participants logged their effort spent using NASA TLX index~\cite{Hart88} (nasatlx.com). We assessed the correctness of a solution by computing the coverage of correct API elements in the solution. We summarize major findings below. More details of the study design and the results are provided in our online appendix~\cite{website:opinerusagemining-online-appendix-ase2018}.

While using our tool, the participants on average coded with more correctness (62\% of all solutions), spent less time (18.6 minutes per task) and less effort (45.8 per task). 
%The difference is statistically significant between our tool and API official documentation based on the effort spent. 
Participants spent the highest amount of time (23.7 minutes) and effort (63.9) per coding solution when using the official documentation. Participants were the least accurate while using Stack Overflow (46\%). After completing the tasks, 29 participants completed a survey to share their experience. 

More than 80\% of the participants considered the mined usage summaries as an improvement over
both API official documentation and Stack Overflow, because our tool offered an increase in productivity, confidence in usage and reduction in time spent. According to one participant:\emt{It is quicker to find solution in [tool] since the subject is well covered and useful information is collected.} 
The participants considered that learning an API could be quicker while using our tool than while using official documentation or Stack Overflow, because our tool synthesizes the information from Stack Overflow by APIs using both sentiment and source code analyses. 

Out of the participants, 87.1\% wanted to use our tool either daily in their development
tasks, or whenever they have specific needs (e.g., learning a new API). All the participants (100\%) rated our tool as usable  for being a single platform to provide insights about API usage and being focused towards a targeted audience. The developers praised the usability, search, and analytics-driven approach in the tool. According to one participant:
\emt{In depth knowledge plus the filtered result can easily increase the productivity of daily development tasks, as it recommends most recently asked questions from Stack Overflow with the quick glimpse of the positive and negative feedback.} As a future improvement, the developers wished our tool to mine usage scenarios from multiple online forums.



% \begin{table}[t]
%   \centering
%   \caption{Distribution of Code Snippets By APIs}
%   %\vspace{-2mm}
%     \begin{tabular}{rrrr|rrrr}\toprule
%     \multicolumn{4}{c}{\textbf{Overall}} & \multicolumn{4}{c}{\textbf{Top 5}} \\
%     \midrule
%     {\textbf{API}} & {\textbf{Snippet}} 
%     & {\textbf{Avg}} & {\textbf{STD}} 
%     & {\textbf{Snippet}} & {\textbf{Avg}} 
%     & {\textbf{Max}} & {\textbf{Min}} \\
%     \midrule
%     175   & 8596  & 49.1  & 502.7 & 5196  & 1039.2 & 1951  & 88    \\
%     \bottomrule
%     \end{tabular}%
%   \label{tbl:api-resolution-overview}%
%   %\vspace{-5mm}
% \end{table}%
% 
% In \tbl\ref{tbl:api-resolution-overview}, we show the distribution of code
% snippets matched to APIs %by the associated APIs 
% using our proposed algorithm. The 8596 code examples are associated with 175
% distinct APIs. The majority of the code examples (60\%) were associated to five
% APIs for parsing JSON-based files and texts in Java: java.util, org.json,
% com.google.code.gson, org.fasterxml.jackson, java.io.
% 
% %\subsubsection{Approach}
% For each of the top five
% APIs, we crawled the online Javadocs and official tutorial pages. We found Javadocs for each API. We did not find any
% tutorial for three APIs (java.util, org.json, and java.io). For each API, we
% computed the coverage of each of the following five API types in the tutorials
% (when available) and the mined usage scenarios:
% \begin{inparaenum}
% \item Class,
% \item Interface,
% \item Annotation,
% \item Exception, and
% \item Enum.
% \end{inparaenum}
% 
% In \tbl\ref{tab:coverage-type-official-mined}, we show the
% coverage of the API types in both official documentation and the mined usage
% scenarios of the five APIs. For each API and for each of the five API types, the
% mined usage scenarios offer more coverage than the official documentation. The
% last column in \tbl\ref{tab:coverage-type-official-mined} shows the overall
% coverage of the API types in the mined vs official documentation. The overall
% coverage is the highest (81.8\%) for the \api{com.google.code.gson} API in the
% mined usage scenarios, followed by 62.5\% in the \api{org.json} API. The
% \api{org.json} API does not have any official tutorial page.
% \begin{table}[t]
% \centering
% \caption{The coverage of API types in the mined usage scenarios and
% in the code examples of API official tutorials (C = Class, I =
% Interface, A = Annotation, EX = Exception, EN = Enum) }
% \vspace{-2mm}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{llrrrrr|r}\toprule
% {\textbf{API}} & \textbf{Resource} & {\textbf{C}}
% & {\textbf{I}} & {\textbf{A}} & {\textbf{EX}}
% & {\textbf{EN}} & {\textbf{Total}} \\
% \midrule
% \multirow{2}[0]{*}{\textbf{java.util}} & Official & 0     & 0     & -     & 0     & -     & 0 \\
% & Mined & 22.22 & 5.26  & -     & 5     & -     & 14.9 \\
% \midrule
% \multirow{2}[0]{*}{\textbf{org.json}} & Official & 0     & 0     & -     & 0
% & -     & 0 \\
% & Mined & 57.14 & 100   & -     & 100   & -     & 62.5 \\
% \midrule
% \multirow{2}[0]{*}{\textbf{gson}} & Official & 28.57 & 75    & 0     & 25    & 0     & 33.33 \\
% & Mined & 85.71 & 87.5  & 50    & 100   & 66.67 & 81.82 \\
% \midrule
% \multirow{2}[0]{*}{\textbf{jackson}} & Official & 1.72  & 0     & 0     & 0     & 20    & 2.21 \\
% & Mined & 5.81  & 4.08  & 34.15 & 44.44 & 12    & 8.5 \\
% \midrule
% \multirow{2}[0]{*}{\textbf{java.io}} & Official & 0     & 0     & -     & 0     & -     & 0 \\
% & Mined & 50.98 & 8.33  & -     & 18.75 & -     & 37.98 \\
% \bottomrule
% \end{tabular}%
% }
% \vspace{-5mm}
% \label{tab:coverage-type-official-mined}%
% \end{table}%
% 
% The two Java official APIs (java.util and java.io) are more of utility types,
% e.g., memory-based collection management of disk-based I/O operations. The APIs
% are not specifically designed for JSON-based features. However, they are among
% the top five APIs, because any JSON-based task may need to perform such
% utility-based operations besides the core task (e.g., JSON parsing).
% Intuitively, the usage scenarios for the two APIs can be mined from other
% threads besides our dataset. Therefore, the coverage of types for the two APIs
% could potentially be much higher in the mined usage scenarios, had we mined all
% the Stack Overflow threads tagged as `Java'.
% 
% The \api{com.fasterxml.jackson} API have the lowest coverage (8.5\%) in the
% mined scenarios. One reason for this is that \api{com.fasterxml.jackson} is the largest API among
% the five APIs in terms of the number of API types. The API has a total of 589
% types (465 classes, 49 interfaces, 41 annotations, 25 enums and 9 exceptions).
% In contrast, the \api{org.json} API has only 16 types (14 classes, 1 interface
% and 1 exception). Therefore, it may happen that developers in our dataset did
% not need to use all of 589 types of the Jackson API. Indeed, Sawant and
% Bacchelli~\cite{Sawant-FineGrapeAPIUsageExtractor-EMSE2016} observed that most
% of the features of an API in Github acturally remain unused by the developers.
% Another possible reason for the lower coverage is that we may have missed the
% discussions of this API in other posts that we did not mine. Our dataset
% consists of all the threads tagged as `Java+JSON'. Not all the Stack Overflow
% threads discussing the usage of the API are tagged as `Java+JSON'. For example,
% the thread (id 27952472) is tagged as `Jackson+java-time'.
% 

